Dynamic Programming Encoding for Subword Segmentation in Neural Machine Translation

This paper introduces Dynamic Programming Encoding (DPE), a new segmentation algorithm for tokenizing sentences into subword units. We view the subword segmentation of output sentences as a latent variable that should be marginalized out for learning and inference. A mixed character-subword transformer is proposed, which enables exact log marginal likelihood estimation and exact MAP inference to find target segmentations with maximum posterior probability. DPE uses a lightweight mixed character-subword transformer as a means of pre-processing parallel data to segment output sentences using dynamic programming. Empirical results on machine translation suggest that DPE is effective for segmenting output sentences and can be combined with BPE dropout for stochastic segmentation of source sentences. DPE achieves an average improvement of 0.9 BLEU over BPE (Sennrich et al., 2016) and an average improvement of 0.55 BLEU over BPE dropout (Provilkov et al., 2019) on several WMT datasets including English <=> (German, Romanian, Estonian, Finnish, Hungarian).

==> fig-raml.tex <==
%%%%%%%%%%%%%%%
\begin{figure*}[h]
    \centering
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.40\textwidth}
        \includegraphics[width=\textwidth]{figures/en-de.png}
        %\caption{A tiger}
        %\label{fig:tiger}
    \end{subfigure}
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.40\textwidth}
        \includegraphics[width=\textwidth]{figures/en-fi.png}
        %\caption{A mouse}
        %\label{fig:mouse}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\textwidth}
        \includegraphics[width=\textwidth]{figures/en-ro.png}
        %\caption{A mouse}
        %\label{fig:mouse}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\textwidth}
        \includegraphics[width=\textwidth]{figures/en-et.png}
        %\caption{A mouse}
        %\label{fig:mouse}
    \end{subfigure}
    \caption{BLEU scores of bpe2bpe model with different settings. ls indicates label smoothing}
    \label{fig:bpe2bpe}
\end{figure*}

==> tab2-oracle.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|cc}
    
           &  \dy (majority) & \dy (oracle)\\
              \midrule
    % WMT &&\\
      Fi-En & 19.18~($\pm$0.23)  &\textbf{19.38}~($\pm$0.11) \\
      En-Fi & 16.57~($\pm$0.05) & \textbf{16.86}~($\pm$0.11) \\
      Ro-En &   31.43~($\pm$0.09) & \textbf{31.50}~($\pm$0.26) \\
      En-Ro &  27.74~($\pm$0.23) & \textbf{28.20}~($\pm$0.04)  \\
      De-En & 31.67~($\pm$0.12)  &\textbf{32.19}~($\pm$0.09) \\
      En-De &  28.27~($\pm$0.05) & \textbf{28.59}~($\pm$0.12)\\
      Et-En & 23.96~($\pm$0.07)  &\textbf{24.21}~($\pm$0.06)  \\
      En-Et &18.36~($\pm$0.03) & \textbf{18.68}~($\pm$0.06)  \\
      \bottomrule
    \end{tabular}
    \caption{BLEU scores among different segmentation pre-processing (WMT).}
    \label{tab:seg-mt}
\end{table}

==> tab3-dropout.tex <==
\begin{table*}[h]
\begin{center}
    \begin{tabular}{l|cccccc}
       & BPE2BPE & Drop2Drop & Drop2BPE & BPE2Drop & DPE2DPE& Drop2DPE\\
     %\hline\hline
     \midrule
      En-Ro & 27.90 &28.07 & 28.04 &27.94 & 28.16  & 28.66\\
      En-Et & 17.64 &  18.20 & 18.09 & 17.94 &18.52 & 18.80\\
%\hline 
      Ro-En & 31.67 & 32.56 & 32.40  & 31.99 &31.81 & 32.99 \\
      %en-fi & 15.88 &  16.24 & * &16.49 & 16.30 \\
      %fi-en &  19.10 & 19.61 & * & 19.53 & 19.82\\
      Et-En &23.13 & 23.65 & 23.52 & 23.38 & 24.17 & *\\
      \bottomrule
    \end{tabular}
\end{center}
\caption{BLEU scores among different segmentation strategies. {\em Drop} means BPE-Dropout}
\label{tab:dropout}
\end{table*}

%\begin{table}[h]
%\begin{center}
%    \begin{tabular}{c|c|c|c}
%      WMT dataset & BPE2BPE & Drop2Drop &  Drop2DPE\\
%     \hline\hline
%     \qquad en-ro & 27.90 &28.07   & 28.66\\
%     \qquad ro-en & 31.67 & 32.56  & 32.99 \\
%     \qquad en-fi & 15.88 &  16.24 & 16.30 \\
%     \qquad fi-en &  19.10 & 19.61  & 19.82\\
%      \qquad en-et & 17.64 &  17.98  & *\\
%     \qquad et-en &23.13 & 23.66  & *\\
%    \end{tabular}
%\end{center}
%\caption{BLEU scores among different segmentation strategies. {\em Drop} means BPE-Dropout}
%\label{tab:dropout2}
%\end{table}
